FedMABA: Towards Fair Federated Learning through Multi-Armed Bandits Allocation

The increasing concern for data privacy has driven the rapid development of federated learning (FL), a privacy-preserving collaborative paradigm. However, the statistical heterogeneity among clients in FL results in inconsistent performance of the server model across various clients. Server model may show favoritism towards certain clients while performing poorly for others, heightening the challenge of fairness. In this paper, we reconsider the inconsistency in client performance distribution and introduce the concept of adversarial multi-armed bandit to optimize the proposed objective with explicit constraints on performance disparities. Practically, we propose a novel multi-armed bandit-based allocation FL algorithm (FedMABA) to mitigate performance unfairness among diverse clients with different data distributions. Extensive experiments, in different Non-I.I.D. scenarios, demonstrate the exceptional performance of FedMABA in enhancing fairness.

==> proof.tex <==
\section{Proof of Theorem 1}

\noindent \textbf{McDiarmid's Inequality} 

Let \( Z_1, \ldots, Z_m \) be independent random variables and let \( f: \mathcal{Z}^m \rightarrow \mathbb{R} \) be a function satisfying the bounded difference property, i.e., for all \( i \) and for all \( z_1, \ldots, z_m, z'_i \) in \( \mathcal{Z} \),
\[ |f(z_1, \ldots, z_{i-1}, z_i, z_{i+1}, \ldots, z_m) - f(z_1, \ldots, z_{i-1}, z'_i, z_{i+1}, \ldots, z_m)| \leq c_i, \]
where \( c_i \) are non-negative constants. Then, for any \( a > 0 \), the following inequality holds:
\[ \mathbb{P}\left( |f(Z_1, \ldots, Z_m) - \mathbb{E}[f(Z_1, \ldots, Z_m)]| \geq a \right) \leq 2 \exp\left( -\frac{2a^2}{\sum_{i=1}^{m} c_i^2} \right). \]

\noindent \textbf{Hoeffding's Inequality}

Let \( X_1, \ldots, X_n \) be independent random variables with \( X_i \) taking values in the interval \( [a_i, b_i] \) almost surely. Define \( \overline{X} = \frac{1}{n} \sum_{i=1}^{n} X_i \) and let \( \mu = \mathbb{E}[\overline{X}] \). Then, for any \( t > 0 \), the following inequality holds:
\[ \mathbb{P}(|\overline{X} - \mu| \geq t) \leq 2 \exp\left( -\frac{2nt^2}{\sum_{i=1}^{n} (b_i - a_i)^2} \right). \]

\begin{assumption}[Bounded Loss]
    \label{bounded loss}
    W.L.O.G. for client $i$, $\forall \xi_i^m, \xi_i^n$, there exists a constant $c$, such that $\lvert F_i(w, \xi_i^m) - F_i(w, \xi_i^n)\rvert<c$.
\end{assumption}

\begin{definition}[Rademacher Complexity]
    Let $\mathcal{F} = F \circ w \triangleq \{\xi \rightarrow F(w, \xi) \mid w \in \mathcal{W}\}$, for any given dataset of FL $S=(\xi^1, ..., \xi^n)$, the set of loss mappings is denoted as $\mathcal{F}_{\mid S} \triangleq \{(F(\xi^1), ..., F(\xi^n)) \mid F\in \mathcal{F} \}$, the Rademacher Complexity is then defined as follows:
    \begin{align}
        \mathcal{R}(\mathcal{F}_{\mid S}) = \frac{1}{N}\mathbb{E}_{\tau \sim \{\pm 1\}^n}\sup_w\sum_{i=1}^N \frac{1}{n_i}\sum_{j=1}^{n_i}\tau F_i(\xi_i^j),
    \end{align}
    where \(\tau\) has an equal probability of 0.5 of being either 1 or -1.
\end{definition}

\begin{definition}[Representation of Generalization Error]
Given the data distribution \( D \) and the training data \( S \), the representation of generalization error is defined as the supremum of the difference between the expected risk and the empirical risk over the hypothesis space $\mathcal{W}$. Formally, it is expressed as:
\begin{align}
    Rep_D(S; \mathcal{W}, \mathcal{F}) = \sup_{w \in \mathcal{W}} (F_D(w) - F_S(w)), 
\end{align}
where $F_{\mathcal{D}}(w)=\mathbb{E}_{\tilde{\xi} \sim\mathcal{D}}F(w, \tilde{\xi})$, and $F_S(w) = \frac{1}{\lvert S \rvert} \sum_{\xi \in S} F(w, \xi)$.

\end{definition}

\begin{lemma}
    \label{empirical}
    Consider a data distribution $\mathcal{D}$ and any train set $S$. $\mathbb{E}_{S \sim D}Rep_{\mathcal{D}(S; \mathcal{F})} \leq 2\mathbb{E}_{S \sim D}R(\mathcal{F_{\mid S}})$.
\end{lemma}

\begin{proof}
   Given any dataset $S=(\xi_1, \xi_2, ..., \xi_n) \sim \mathcal{D}$, $S'=(\xi_1^{'}, \xi_2^{'}, ..., \xi_n^{'}) \sim D $. 
\[
\begin{aligned}
    \mathbb{E}_S Rep_{\mathcal{D}}(S; \mathcal{W}, \mathcal{F})
    &= \mathbb{E}_S \left[ \sup_{w \in \mathcal{W}} \{ F_{\mathcal{D}}(w) - F_{\mathcal{S}}(w) \} \right], \\
    &= \mathbb{E}_S \left[ \sup_{w \in \mathcal{W}} \{ \mathbb{E}_{S'} [F_{S'}(w)] - F_{S}(w) \} \right], \\
    &= \mathbb{E}_{S,S^{'}}\operatorname*{sup}_{w\in\mathcal{W}}\{\frac{1}{n}\sum_{i=1}^{n}(F(\xi_{i}^{\prime})-F(\xi_{i}))\}, \\
    &= \mathbb{E}_{S,S^{'},\tau\sim\{\pm1\}^n}\sup_{w\in\mathcal{W}}\{\frac1n\sum_{i=1}^n(\tau_iF(\xi_i^{\prime})-\tau_iF(\xi_i))\}, \\
    &\leq\mathbb{E}_{S^{\prime},\tau}\sup_F\{\frac1n\sum_{i=1}^n\tau_iF(\xi_i^{\prime})\}+\mathbb{E}_{S,\tau}\sup_F\{\frac1n\sum_{i=1}^m\tau_iF(\xi_i)\}, \\
    &= 2R(\mathcal{F_{\mid S}})
\end{aligned}
\] 
\end{proof}




% \begin{lemma}
%     \label{lemma 1}
%     Assume $\forall \xi_m, \xi_n$, $\lvert F_i(w, \xi_m) - F_i(w, \xi_n)\rvert<c$. Define $ \text{Rep}(\mathcal{H}, S) \triangleq \sup_{w \in \mathcal{H}} \left(F_i(w, \xi_m) - \hat{F}_i(w)  \right), $ where $\mathcal{H}$ is the parameter hypothesis set and \( S \) is the sample space, then for $\forall \delta \in \left[0, 1\right]$, with probability of at least $1-\delta$:
%     \begin{align}
%         Rep(\mathcal{H},S)\leq\mathbb{E}_SRep(\mathcal{H},S)+c\sqrt{\frac{2\ln(2/\delta)}{N}}
%     \end{align}
% \end{lemma}

% \begin{lemma}
%     Define
%     \begin{align}
%         R(\mathcal{F}|_{S}) \triangleq \frac{1}{N}\mathbb{E}_{\tau\sim\{\pm1\}^{n_i}}\sup_{w}
%         \sum_{i=1}^N \frac{1}{n_i}\sum_{j=1}^{n_i}\tau_{i, j}F_i(w_i, \xi_j) .
%     \end{align}
%     Combine Lemma \ref{lemma 1}, for $\forall \delta \in \left[0, 1\right]$, with probability of at least $1-2\delta$:
%     \begin{align}
%         \frac{1}{N}\sum_{i=1}^N(F_i(w_i)-\hat{F}_i(w_i)) \leq 2 R(\mathcal{F}|_{S}) + 3c\sqrt{\frac{2\ln(2/\delta)}{N}}
%     \end{align}
% \end{lemma}

\begin{theorem}[Bounded Generalization Error]
    \label{bounded generalization error}
    Consider a FL system with N clients, and parameter hypothesis space $\mathcal{W}$. If Assumption \ref{bounded loss} holds. Then, for $\forall \delta \in \left[0, 1\right]$ with probability of at least $1-2\delta$, for $\forall w \in \mathcal{W}$, the generalization error can be upper bounded as:
    \begin{align}
        Rep_D(S; \mathcal{W}, \mathcal{F}) \leq 2\mathcal{R}(\mathcal{F}_{\mid S}) + 3c\sqrt{\frac{2\ln \frac{2}{\delta}}{N}}.
    \end{align}
\end{theorem}

\begin{proof}
    Let's start with McDiarmid's Inequality, let $f(S)=Rep_D(S;\mathcal{F})$, we have 
    \begin{align}
        \mathbb{P}\left(\mathrm{Rep}_{\mathcal{D}}(S;\mathcal{F})-\mathbb{E}[\mathrm{Rep}_{\mathcal{D}}(S;\mathcal{F})]\geq\epsilon\right)\leq 2\exp\left(-\frac{2\epsilon^2}{mc^2}\right).
    \end{align}
    Set $\delta=\exp{(-\frac{2\epsilon^2}{Nc^2})}$, we then have
    \begin{align}
        \epsilon=c\sqrt{\frac{2\ln(2/\delta)}N}, 
    \end{align}
    Next, we consider empirical Rademacher complexity.
    According to \ref{empirical}, with a probability of at least $1-\delta$, we can obtain 
    \begin{align}
        \label{combine1}
        Rep_{\mathcal{D}}(S;\mathcal{F})\leq2\mathbb{E}_{S}R(\mathcal{F}|_{S})+c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}
    Then consider $\mathbb{E}_{S}R(\mathcal{F}|_{S})$, given $c^\prime = \frac{c}{2}\sqrt{N}$, with a probability of at least $1-\delta$, we have
    \begin{align}
        \label{combine2}
        \mathbb{E}_SR(\mathcal{F}|_S)\leq R(\mathcal{F}|_S)+c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}
    Combine \ref{combine1} and \ref{combine2}, and thus with a probability of at least $1-2\delta$, we have
    \begin{align}
        Rep_{\mathcal{D}}(S;\mathcal{F})\leq2R(\mathcal{F}|_{S})+3c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}
\end{proof}


\begin{corollary}[Bounded Generalization Error]
    \label{extended theorem}
     Under the same conditions as Theorem \ref{bounded generalization error}, let S, D be the training set and generalization data distribution, $w_S = ERM_w(S) = argmin_{w\in \mathcal{W}}{F(w;S)}$, $w^* = argmin_{w\in \mathcal{W}}{F(w;D)}$. Then, for $\forall \delta \in \left[0, 1\right]$ with probability of at least $1-3\delta$, for $\forall w \in \mathcal{W}$, the generalization error can be bounded as:
    \begin{align}
        F_{\mathcal{D}}(w_S)-F_{\mathcal{D}}(w^*)\leq 2\sup_{w \in \mathcal{W}} Var(F)+4c\sqrt{\frac{2\ln(2/\delta)}{N}}, 
    \end{align} 
    where $Var(F) = \sqrt{\frac{1}{N}\sum_{i=1}^{N}(F_{i}(w)-\frac{1}{N}\sum_{i=1}^{N}F_{i}(w))^2}$.
\end{corollary}

\begin{proof}
    Denote $w_S, w^*$ as $w_S=ERM_{\mathcal W}(S)=\arg\min_{w\in\mathcal W}\{F_S(w)\}, w^*=\arg\min_{w\in\mathcal W}\{F_D(w)\}$.
    Then we can rewrite generalization error as
    \begin{align}
        &F_{\mathcal{D}}(w_{S})-F_{\mathcal{D}}(w^{*})=\underbrace{[F_{\mathcal{D}}(w_{S})-F_{S}(w_{S})]}_{P_1}+\underbrace{[F_{S}(w_{S})-F_{S}(w^{*})]}_{P_2}+\underbrace{[F_{S}(w^{*})-F_{\mathcal{D}}(w^{*})]}_{P_3}.
    \end{align}

    \begin{align}
        \label{P1}
        P_1 &= F_{\mathcal{D}}(w_{S})-F_{S}(w_{S}) \\
        & \leq Rep_{\mathcal{D}}(S;\mathcal{F})\leq^{1-2\delta}2R(\mathcal{F}|_{S})+3c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}

    \begin{align}
        \label{P2}
        P_2 &= F_{S}(w_{S})-F_{S}(w^{*}) \\
        & \leq0.
    \end{align}

    According to the McDiarmid's inequality.
    \begin{align}
        \label{P3}
        F_{S}(w^{*})-F_{\mathcal{D}}(w^{*})\leq^{1-\delta}\frac{2c}{\sqrt{m}}\sqrt{\frac{m\ln(2/\delta)}{2}}.
    \end{align}

    Combining \ref{P1} to \ref{P3}, and following \cite{yuan2023equitable}, with a probability of at least $1-3\delta$, we obtain
    \begin{align}
        F_{\mathcal{D}}(w_S)-F_{\mathcal{D}}(w^*)\leq2\sup\limits_{w\in\mathcal{W}}Var(F)+4c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}    
\end{proof}

\section{Derivations of the Update Rule for the Player}
We mainly refer \cite{mao2021banditmtl} to the iterative derivation of $p$. We introduce the Legendre function related to $p$ as $\Phi_p(p)=\sum_{i=1}^Np_i\log p_i$. Assume the mirror gradient ascent step $t+1$, without loss of generality, in the dual space is $q^{t+1}$. The mirror gradient ascent step of the dual space can be defined as follows:
\begin{align}
    \label{all nabla}
    \nabla\Phi_p(q^{t+1})=\nabla\Phi_p(p^t)+\eta_b\mathbf{F}(w^t) ,
\end{align}
where $\mathbf{F}(w^t)$ denotes the loss vector of all participants, $\eta_b$ is the step size of the dual space, also known as MAB step size in main paper. For any client $i$, the corresponding $i$-th element of $\nabla\Phi_p(q^{t+1})$ is:
\begin{align}
    \label{element nabla}
    \nabla\Phi_p(q_i^{t+1})=1+\log q_i^{t+1} .
\end{align}
Combining \ref{all nabla} and \ref{element nabla}, the representational relationship between $q$ and $p$ is deduced as:
\begin{align}
    \label{q}
    q_i^{t+1}=e^{(\nabla\Phi_p(p_i^t)+\eta_bF_i(w_i^t)-1)}.
\end{align}
After updating the dual space weights $q^t$, in order to map them back to the original problem space to get update of $p^t$, we need to solve the following problem:
\begin{align}
    \label{map back}
    p^{t+1}=\arg\min_{p\in\mathcal{P}_{\rho,\mathbf{N}}}D_{\Phi_{p}}(p,q^{t+1}) ,
\end{align}
where $D_{\Phi_{p}}(p,q^{t+1}) = \Phi_p(p)-\Phi_p(q^{t+1})-\langle\nabla\Phi_p(q^{t+1}),p-q^{t+1}\rangle $ is the Bregman Divergence.

Incorporating the constraints of $p$, we establish the Lagrangian function as follows:
\begin{align}
&F(p^{t+1},\beta,\lambda)=\sum_{i=1}^{N}p_{i}^{t+1}\log\frac{p_{i}^{t+1}}{q_{i}^{t+1}} \nonumber \\ 
&- \beta(\sum_{i=1}^Np_i^{t+1}-1)-\lambda(\rho-\sum_{i=1}^Np_i^{t+1}\log p_i^{t+1}N).
\end{align}
Using the first order conditions, we have
\begin{align}
    p_i^{t+1}=(q_i^{t+1})^{\frac{1}{1+\lambda}}N^{-\frac{\lambda}{1+\lambda}}\exp(\frac{\alpha}{1+\lambda}-1).
\end{align}
Combining with $\sum_{i=1}^{N}p_{i}^{t+1}=1$, the constant part can be replaced by 
\begin{align}
    N^{-\frac\lambda{1+\lambda}}\exp\left(\frac\alpha{1+\lambda}-1\right)=\frac1{\sum_{i=1}^N(q_i^{t+1})^{\frac1{1+\lambda}}}, 
\end{align}
and then we have
\begin{align}
    \label{p iter}
    p_i^{t+1}=(q_i^{t+1})^{\frac{1}{1+\lambda}}/(\sum_{i=1}^N(q_i^{t+1})^{\frac{1}{1+\lambda}}).
\end{align}
By substituting \ref{p iter} back into the Lagrangian function and taking the derivative with respect to lambda, we have
\begin{align}
    \label{lambda diff}
    \frac{d}{d\lambda}\mathcal{L}(\lambda)&=\log N-\rho-\log\sum_{i=1}^N(q_i^{t+1})^{\frac1{1+\lambda}}\nonumber \\&- \frac{\sum_{i=1}^Nlog(q_i^{t+1})(q_i^{t+1})^{\frac1{1+\lambda}}}{(1+\lambda)\sum_{i=1}^N(q_i^{t+1})^{\frac1{1+\lambda}}}.
\end{align}
Combining \ref{lambda diff} and \ref{q}, the update formula for $p$ can be expressed as
\begin{align}
    p_i^{t+1}=\frac{e^{\frac{1}{1+\lambda^*}(\log p_i^t+\eta_bF_i(w^t_i)}}{\sum_{i=1}^Ne^{\frac{1}{1+\lambda^*}(\log p_i^t+\eta_bF_i(w^t_i)}}, 
\end{align}
where $\lambda^*$ is the kernel of $\frac{d}{d\lambda}\mathcal{L}(\lambda)$ which is denoted as $f(\lambda)$ in the main paper.

\section{Convergence of FedMABA}

\noindent Recall the assumptions we've made to derivate the convergence of FedMABA:
\begin{assumption}[Smoothness]
    \label{ass 1}
    Each objective function of clients is Lipschitz smooth, that is, there exists a constant $L > 0$, such that $\|\nabla F_i(\boldsymbol{x})-\nabla F_i(\boldsymbol{y})\|\leq L\left\|\boldsymbol{x}-\boldsymbol{y}\right\|,\forall i\in\{1,2,\ldots,N\}.$
\end{assumption}

\begin{assumption}[Unbiased Gradient and Bounded clients' Variance]
    \label{ass 2}
    The stochastic gradient calculated by each client can be an unbiased estimator of the clients' gradient $\mathbb{E}_\xi[g_i(\boldsymbol{p^{avg}}|\xi)]=\nabla F_i(\boldsymbol{p^{avg}}),$ and has bounded variance $\mathbb{E}_\xi[\|g_i(\boldsymbol{p^{avg}}|\xi)-\nabla F_i(\boldsymbol{p^{avg}})\|^2]\leq\sigma^2,\forall i\in\{1,2,\ldots,N\},\sigma^2\geq0.$
\end{assumption}

\begin{assumption}[Bounded Dissimilarity of Clients' Gradient]
    \label{ass 3}
    For any sets of weights $\{p_{i}^t\geq0\}_{i=1}^{N},\sum_{i=1}^{N}p_{i}^t=1,$, there exist constants $(\gamma^2+1) \geq 1$, $A^2 \geq 1$, such that $\sum_{i=1}^Np_i^t\left\|\nabla F_i(\boldsymbol{p^{avg}})\right\|^2\leq\gamma^2\left\|\sum_{i=1}^Np_i^t\nabla F_i(\boldsymbol{p^{avg}})\right\|^2+A^2.$
\end{assumption}

\begin{assumption}[Bounded Weights Divergence]
    \label{ass 4}
    For any sets of weights $p^t$ derived by FedMABA, $\chi_{p^a\|p^t}^{2}$, the chi-square divergence of $p^t$ and the average weights $p^a = \left[\frac{1}{N}, ..., \frac{1}{N}\right]$ can be upper bounded by $\kappa$, that is, $\forall t = 1, ..., T$, there exists a constant $\kappa$, such that $\chi_{p^a\|p^t}^{2} \leq \kappa$, where $\chi^2_{{p^a}\|{p^t}}=\sum_{i=1}^N\left(p^a_i-p^t_i\right)^2/p^t_i$.     
\end{assumption}


\noindent We first explain the gradient differences caused by the aggregation probability bias, following \cite{wang2020tackling}.

\begin{lemma}[Including bias in the error bound.]
    For any model parameter $w$, the difference between the gradients of $F^{avg}(w)=\sum_{i=1}^N p^{avg}_i F_i(w_i)$ and $F(w)=\sum_{i=1}^N p_i F_i(w_i)$ can be bounded as follows:
\begin{align}
    \|\nabla f^{avg}(w)-\nabla f(w)\|^2 \leq \chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2\left[(\gamma^2-1)\|\nabla {f}(w)\|^2+A^2 \right] \, ,
\end{align}
where $\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2$ denotes the chi-square distance between $\boldsymbol{p^{avg}}$ and $\boldsymbol{p}$, i.e., $\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2=\sum_{i=1}^N\left(p^{avg}_i-p_i\right)^2 / p_i$. $f(x)$ is the global objective with $f(w)=\sum_{i=1}^Np_if_i(w)$ where $\boldsymbol{p^{avg}}$ is usually the data ratio of clients. ${f}(w)=\sum_{i=1}^{N}p_if_i(w)$ is the  objective function of FedMABA with the reweight aggregation probability $\boldsymbol{p}$.
\label{objective gap}
\end{lemma}

\begin{proof}

\begin{equation}
\begin{aligned}
\nabla f^{avg}(x)-\nabla  {f}(\boldsymbol{x}) & =\sum_{i=1}^N\left(p^{avg}_i-p_i\right) \nabla f^{avg}_i(w) \\
& =\sum_{i=1}^N\left(p_i^{avg}-p_i\right)\left(\nabla f^{avg}_i(w)-\nabla  {f}(w)\right) \\
& =\sum_{i=1}^M \frac{p_i^{avg}-p_i}{\sqrt{p}_i} \cdot \sqrt{p}_i\left(\nabla f^{avg}_i(w)-\nabla {f}(w)\right) \, .
\end{aligned}
\end{equation}

Applying Cauchy-Schwarz inequality, it follows that
\begin{equation}
\begin{aligned}
\|\nabla f^{avg}(w)-\nabla {f}(w)\|^2 & \leq\left[\sum_{i=1}^N \frac{\left(p^{avg}_i-p_i\right)^2}{p_i}\right]\left[\sum_{i=1}^N p_i\left\|\nabla f^{avg}_i(w)-\nabla {f}(w)\right\|^2\right] \\
& \leq \chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2\left[(\gamma^2-1)\|\nabla {f}(w)\|^2+A^2\right] \, ,
\end{aligned}
\end{equation}
where the last inequality uses Assumption~\ref{ass 3}.
Note that
\begin{equation}
\begin{aligned}
\|\nabla f^{avg}(w)\|^2 & \leq 2\|\nabla f^{avg}(w)-\nabla {f}(w)\|^2+2\|\nabla {f}(w)\|^2 \\
& \leq 2\left[\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1\right]\|\nabla {f}(w)\|^2+2 \chi_{\boldsymbol{p^{avg}}\| \boldsymbol{p}}^2  A^2 \, .
\end{aligned}
\end{equation}

As a result, we obtain

\begin{align}
\min _{t \in[T]}\left\|\nabla f^{avg}\left(w^t\right)\right\|^2 & \leq \frac{1}{T} \sum_{t=0}^{T-1}\left\|\nabla f^{avg}\left(w^t\right)\right\|^2   \\
& \leq 2\left[\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1\right] \frac{1}{T} \sum_{t=0}^{T-1}\left\|\nabla {f}\left(w^t\right)\right\|^2+2 \chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2 A^2  \\
& \leq 2\left[\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1\right] \epsilon_{\mathrm{opt}}+2 \chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2 A^2 \, ,
\label{global convergence}
\end{align}
where $\epsilon_{\mathrm{opt}}= \frac{1}{T} \sum_{t=0}^{T-1}\left\|\nabla {f}\left(w^t\right)\right\|^2$ denotes the optimization error.
\end{proof}


\noindent Following \cite{wang2023delta}, we present the following convergence analysis.
\begin{lemma}[Local updates bound.]
    For a sufficiently small client's step size $\eta_c \leq \frac{1}{8LK}$, the local updates can be bounded as:
    \begin{align}
        \mathbb{E}\|w_{i,k}^t-w^t\|^2\leq20K^2(\eta_c^2\sigma^2+\eta_c^2A^2 + \gamma^2\eta_c^2\|\nabla F(x^t)\|^2).
    \end{align}
\end{lemma}

\begin{proof}

\begin{align}
    \mathbb{E}_t \|w_{i,k}^t-w^t\|^2 & = \mathbb{E}_t\|w_{i,k-1}^t-w^t-\eta_cg_{i,k-1}^t\|^2 \\
    & = \mathbb{E}_t\|w_{i,k-1}^t-w^t-\eta_c ( g_{i,k-1}^t-\nabla F_i(w_{i,k-1}^t)+\nabla F_i(w_{t,k-1}^t) -\nabla F_i(w^t)+\nabla F_i(w^t) ) \|^2 \\
    &\leq (1+\frac{1}{2K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\mathbb{E}_t\|\eta_c(g_{i,k-1}^t-\nabla F_i(w_{i,k}^t))\|^2 \notag \\
    &\quad +2K \mathbb{E}_t[\|\eta_L(\nabla F_i(w_{i,K-1}^t)-\nabla F_i(w^t))\|^2] + 2K\eta_c^2\mathbb{E}_t\|\nabla F_i(w^t)\|^2 \\
    &\leq (1+\frac{1}{2K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\eta_c^2\sigma^2 + 2K\eta_c^2L^2\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 \notag \\
    &\quad + 2K\eta_c^2A^2 + 2K\gamma^2\|\eta_c\nabla f(w^t)\|^2 \\
    &\leq (1+\frac{1}{K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\eta_c^2\sigma^2 + 2K\eta_c^2A^2 + 2K\gamma^2\|\eta_c\nabla F(w^t)\|^2 . 
\end{align}

By recursively applying the above formula, we can obtain,
\begin{align}
\mathbb{E}_t\|w_{i,k}^t-w^t\|^2 &\leq \sum_{p=0}^{k-1}(1+\frac{1}{K-1})^p\left[4K\eta_c^2\sigma^2+4K\eta_c^2A^2+4K\gamma^2\|\eta_c\nabla {F}(w^t)\|^2\right]  \\
&\leq (K-1)\left[(1+\frac{1}{K-1})^K-1\right]\left[4K\eta_c^2\sigma^2+4K\eta_c^2A^2+4K\gamma^2\|\eta_c\nabla {F}(w^t)\|^2\right]  \\
&\leq 20K^2(\gamma^2\eta_c^2\|\nabla {F}(w^t)\|^2 +\eta_c^2\sigma^2+\eta_c^2A^2)\, .
\end{align}
\end{proof}

We thus can formulate the convergence analysis of FedMABA.
\begin{theorem}[Convergence bound]
    Under Assumption \ref{ass 1} to \ref{ass 4}, let $\eta_s, \eta_c$ be the server updating step size, and the clinet's one, respectively. Set $\eta_c$ small enough as $\eta_c < \min (\frac{1}{8LK}, C)$, where C is a constant, such that $\frac{1}{2}-10 L^2\frac{1}{N}\sum_{i=1}^N K^2\eta_c^2\gamma^2(\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2)-1)^2+1) \leq c \leq 0$, and $\eta_s < \frac{1}{\eta_cL}$, the expectation of the gradient norm can be upper bounded when running FedMABA as:
    \begin{align}
    \mathop{min}_{\limits_{t\in[T]}} \mathbb{E}_t \|\nabla F(w^t)\|^2 \leq \frac{F^0-F^*}{c\eta_s\eta_cK T} +\Psi ,
    \end{align}
where 
\begin{align}
   \Psi 
    &= \frac{1}{C} [
     10\eta_c^2K^2L^2(\sigma^2 + A^2) + \frac{\eta_s\eta_c L}{2}\sigma^2 +20L^2K^2\gamma^2\eta_c^2\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2] \, .
\end{align}
where $\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2=\sum_{i=1}^N\left(p_i^{avg}-p_i\right)^2 / p_i$ represents the chi-square divergence between the average aggragation weights $p^{avg}$ and the MAB aggregation weights $p$.
\end{theorem}

\begin{proof}
    \begin{align}
& E_t[{F}(w^{t+1})] \\
& \leq {F}(w^t) + \left \langle \nabla  {F}(w^t),E_t[w^{t+1}-w^t] \right \rangle + \frac{L}{2}E_t[\left \| w^{t+1}-w^t \right \|^2]  \\
&= {F}(w^t)+\left \langle \nabla  {F}(w^t),E_t[\eta_s \Delta_t+\eta_s\eta_c K\nabla  {F}(w^t)-\eta_s\eta_c K \nabla  {F}(w^t)] \right \rangle+\frac{L}{2}\eta_s^2E_t[\left \|\Delta_t \right \|^2]  \\
&=  {F}(w^t)-\eta_s\eta_c K\left \|\nabla  {F}(w^t)\right \|^2 + \eta_s\underbrace{\left \langle \nabla  {F}(w^t), E_t[\Delta_t+\eta_c K\nabla  {F}(w^t)] \right\rangle}_{P_1}+\frac{L}{2}\eta_s^2\underbrace{E_t\|\Delta_t\|^2}_{P_2} \, ,
\end{align}

\begin{align}
    &\ P_1 
    =\left \langle \nabla  {F}(w^t),E_t[\Delta_t+\eta_cK\nabla  {F}(w^t)]\right\rangle   \\
    &=\left \langle \nabla  {F}(w^t),E_t[-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\eta_cg_{i,k}^t+\eta_cK\nabla  {F}(w^t)]\right\rangle  \\
    &=\left \langle \nabla  {F}(w^t),E_t[-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\eta_c\nabla F_i(w_{i,k}^t)+\eta_cK\nabla  {F}(w^t)]\right\rangle  \\
    &=\left \langle \sqrt{\eta_cK}\nabla  {F}(w^t),-\frac{\sqrt{\eta_c}}{\sqrt{K}}E_t[\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}(\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t))]\right\rangle  \\
    &=\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2K}E_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}(\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t)) \right\|^2   \notag \\
    &\ ~~~~ - \frac{\eta_c}{2 K}E_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \\
    &\leq\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2}\sum_{k=0}^{K-1}\sum_{i=1}^Np^{avg}_i\mathbb{E}_t\left\|\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t) \right\|^2  \notag \\
    &\ ~~~~- \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
     &\leq\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_cL^2}{2N}\sum_{i=1}^N\sum_{k=0}^{K-1}\mathbb{E}_t\left\|w_{i,k}^t-w^t \right\|^2 - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
    &\leq \left(\frac{\eta_cK}{2}+10K^3L^2\eta_c^3\gamma^2\right)\|\nabla  {F}(w^t)\|^2 + 10L^2\eta_c^3K^3\sigma^2+  10\eta_c^3L^2K^3A^2  \notag \\ 
    &\ ~~~~ - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \, ,
\end{align}

\begin{align}
    &\ P_2 
    =\mathbb{E}_t\|\Delta_t\|^2   \\
    &=\mathbb{E}_t\left\|\eta_c\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}g_{i,k}^t\right\|^2   \\
    &=\eta_c^2\mathbb{E}_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}g_{i,k}^t-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2 +\eta_c^2\mathbb{E}_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2   \\
    &\leq \eta_c^2\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\mathbb{E}\|g_i(w_{i,k}^t)-\nabla F_i(w_{i,k}^t)\|^2 +\eta_c^2\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
    & \leq \eta_c^2K\sigma^2 
    + \eta_c^2 \mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2    \, .
\end{align}
Now we take expectation over iteration on both sides of expression:
\begin{align}
    & \ F(w^{t+1}) \\
    &\leq F(w^t)-\eta_s\eta_cK\mathbb{E}_t\left \|\nabla  {F}(w^t)\right \|^2 + \eta_s\mathbb{E}_t\left \langle \nabla  {F}(w^t),\Delta_t+\eta_cK\nabla  {F}(w^t) \right\rangle +\frac{L}{2}\eta_s^2\mathbb{E}_t\|\Delta_t\|^2   \\
    &\leq F(w^t) -\eta_s\eta_cK\left(\frac{1}{2}-20 L^2 K^2\eta_c^2\gamma^2(\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1) \right)\mathbb{E}_t\left\|\nabla  {f}(w^t)\right\|^2 
    \notag \\ 
    &\ ~~~~+10\eta_s\eta_c^3L^2K^3(\sigma^2 +A^2)  
    +\frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 + 20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2  \notag \\
    &\ ~~~~ -\left(\frac{\eta_s\eta_c}{2K}-\frac{L\eta_s^2\eta_c^2}{2}\right)\mathbb{E}_t\left\|\frac{1}{N}\sum_{i=1}^N\sum_{k=0}^{K-1}\nabla F_i(x_{i,k}^t)\right\|^2   \\
    &\leq F(w^t) -C\eta_s\eta_cK\mathbb{E}\left\|\nabla  {f}(w^t)\right\|^2 
    +10\eta_s\eta_c^3L^2K^3(\sigma^2 +A^2)    \\
    &\ ~~~~ +\frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 + 20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2  \notag \\
    & \ ~~~~ -\left(\frac{\eta_s\eta_c}{2K}-\frac{L\eta_s^2\eta_c^2}{2}\right)\mathbb{E}_t\left\|\frac{1}{N}\sum_{i=1}^N\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2    \\
    &\leq F(w^t) - c\eta_s\eta_cK\mathbb{E}_t\|\nabla  {F}(w^t)\|^2 +10\eta_s\eta_c^3L^2K^3(\sigma^2 +A^2)  \notag \\
    &\ ~~~~ + \frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 +20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2 \, ,
\end{align}
By recursively summing the the error difference above, we can obtain
\begin{align}
    \sum_{t=1}^{T-1}C\eta_s\eta_cK\mathbb{E}\|\nabla F(w^t)\|^2\leq F(w^0)-F(w^T)+T(\eta_s\eta_cK)\Psi,
\end{align}
where 
\begin{align}
    \Psi 
    &= \frac{1}{C} [
     10\eta_c^2K^2L^2(\sigma^2 + A^2) + \frac{\eta_s\eta_c L}{2}\sigma^2 +20L^2K^2\gamma^2\eta_c^2\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2] \, .
\end{align}

\begin{corollary}
    Suppose $\eta_s$ and $\eta_c$ are $\eta_c=\mathcal{O}\left(\frac{1}{\sqrt{T}KL}\right)$ and $\eta_s=\mathcal{O}\left(\sqrt{KN}\right)$ such that the conditions mentioned above are satisfied. Then for sufficiently large T, the iterates of FedMABA satisfy:
    \begin{align}
        % \min_{t\in[T]}\mathbb{E}\|\nabla F(\boldsymbol{p^{avg}}^{(t)})\|^{2}\leq\mathcal{O}\left(\frac{F^0-F^*}{\sqrt{NKT}}\right)+\mathcal{O}\left(\frac{4\sqrt{N}\sigma^{2}L}{\sqrt{KT}}\right)+ \nonumber \\
        % \mathcal{O}\left(\frac{6NL^2(K-1)\sigma^{2}}{KT}\right)+\mathcal{O}\left(\frac{12NL^2(K-1)A^2}{T}\right) .
        \min_{t\in[T]}\mathbb{E}\left\|\nabla f\left(w\right)\right\|^2\leq\mathcal{O}\left(\frac{1}{\sqrt{NKT}}+\frac{1}{T}\right).
    \end{align}
\end{corollary}


\begin{table}[!t]
    \small
    \caption{\small hyper-parameters of all experimental algorithms.}
    \resizebox{.4\textwidth}{!}{
    \begin{tabular}{ll}
    \toprule
        Algorithm & Hyper Parameters \\ \midrule
        $q-FFL$ &  $q \in \{0.005, 0.01, 0.1, 0.5, 5, 15\}$ \\ 
        $PropFair$ & $M \in \{0.2, 5.0\}, \epsilon = 0.2$ \\
        $AFL$ & $\lambda \in \{0.01, 0.1, 0.5, 0.7\}$ \\ 
        $TERM$ & $T \in \{0.1, 0.5, 0.8\}$ \\ 
        $FedMGDA+$ & $\epsilon \in \{0.1, 1.0\}, \eta=1.0$ \\
        $FedProx$ & $\mu = 0.1 $ \\
        % $Scaffold$ & $\eta = 1.0 $,${\mu = 1.0}$ \\
        \multirow{2}{*}{$FedMABA$} & $\eta_b \in \{1.0, 0.7, 0.5, 0.3, 0.1\}$, \\
        & $\alpha \in \{0.1, 0.3, 0.5, 0.7, 0.9\}, \rho=1.0$ \\ \bottomrule
        % FedEBA & $ T \in \{1.0, 0.5, 0.1, 0.05, 0.01\}$ \\ 
    \end{tabular}
    }
    \centering
    \label{hyper table}
    \vspace{-2.em}

\end{table}
% \begin{align}
%     &\ A_1 \\
%     &\overset{(a4)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2}\sum_{k=0}^{K-1}\sum_{i=1}^Np^{avg}_i\mathbb{E}_t\left\|\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t) \right\|^2  \notag \\
%     &\ ~~~~- \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%      &\overset{(a5)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_cL^2}{2N}\sum_{i=1}^N\sum_{k=0}^{K-1}\mathbb{E}_t\left\|w_{i,k}^t-w^t \right\|^2 - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%     &\leq \left(\frac{\eta_cK}{2}+10K^3L^2\eta_c^3\gamma^2\right)\|\nabla  {F}(w^t)\|^2 + \frac{5L^2\eta_c^3}{2}K^2\sigma^2+  10\eta_c^3L^2K^3A^2  \notag \\ 
%     &\ ~~~~ - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \, ,
% \end{align}
\end{proof}
% \noindent Following \cite{wang2023delta}, we present the following convergence analysis.
% \begin{lemma}[Local updates bound.]
%     For a sufficiently small client's step size $\eta_c \leq \frac{1}{8LK}$, the local updates can be bounded as:
%     \begin{align}
%         \mathbb{E}\|w_{i,k}^t-w^t\|^2\leq5K(\eta_c^2\sigma^2+4K\eta_c^2A^2)+20K^2\gamma^2\eta_c^2\|\nabla F(x^t)\|^2.
%     \end{align}
% \end{lemma}

% \begin{proof}

% \begin{align}
%     \mathbb{E}_t \|w_{i,k}^t-w^t\|^2 & = \mathbb{E}_t\|w_{i,k-1}^t-w^t-\eta_cg_{i,k-1}^t\|^2 \\
%     & = \mathbb{E}_t\|w_{i,k-1}^t-w^t-\eta_c ( g_{i,k-1}^t-\nabla F_i(w_{i,k-1}^t)+\nabla F_i(w_{t,k-1}^t) -\nabla F_i(w^t)+\nabla F_i(w^t) ) \|^2 \\
%     &\leq (1+\frac{1}{2K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\mathbb{E}_t\|\eta_c(g_{i,k-1}^t-\nabla F_i(w_{i,k}^t))\|^2 \notag \\
%     &\quad +2K \mathbb{E}_t[\|\eta_L(\nabla F_i(w_{i,K-1}^t)-\nabla F_i(w^t))\|^2] + 2K\eta_c^2\mathbb{E}_t\|\nabla F_i(w^t)\|^2 \\
%     &\leq (1+\frac{1}{2K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\eta_c^2\sigma^2 + 2K\eta_c^2L^2\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 \notag \\
%     &\quad + 2K\eta_c^2A^2 + 2K\gamma^2\|\eta_c\nabla f(w^t)\|^2 \\
%     &\leq (1+\frac{1}{K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\eta_c^2\sigma^2 + 2K\eta_c^2A^2 + 2K\gamma^2\|\eta_c\nabla F(w^t)\|^2 . 
% \end{align}

% By recursively applying the above formula, we can obtain,
% \begin{align}
% \mathbb{E}_t\|w_{i,k}^t-w^t\|^2 &\leq \sum_{p=0}^{k-1}(1+\frac{1}{K-1})^p\left[4K\eta_c^2\sigma^2+4K\eta_c^2A^2+4K\gamma^2\|\eta_c\nabla {F}(w^t)\|^2\right]  \\
% &\leq (K-1)\left[(1+\frac{1}{K-1})^K-1\right]\left[4K\eta_c^2\sigma^2+4K\eta_c^2A^2+4K\gamma^2\|\eta_c\nabla {F}(w^t)\|^2\right]  \\
% &\leq 20K^2(\gamma^2\eta_c^2\|\nabla {F}(w^t)\|^2 +\eta_c^2\sigma^2+\eta_c^2A^2)\, .
% \end{align}
% \end{proof}

% We thus can formulate the convergence analysis of FedMABA.
% \begin{theorem}[Convergence bound]
%     Under Assumption \ref{ass 1} to \ref{ass 4}, let $\eta_s, \eta_c$ be the server updating step size, and the clinet's one, respectively. Set $\eta_c$ small enough as $\eta_c < \min (\frac{1}{8LK}, C)$, where C is a constant, such that $\frac{1}{2}-10 L^2\frac{1}{N}\sum_{i=1}^N K^2\eta_c^2\gamma^2(\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2+1) \leq c \leq 0$, and $\eta_s < \frac{1}{\eta_cL}$, the expectation of the gradient norm can be upper bounded when running FedMABA as:
%     \begin{align}
%     \mathop{min}_{\limits_{t\in[T]}} \mathbb{E}_t \|\nabla F(w^t)\|^2 \leq \frac{F^0-F^*}{c\eta_s\eta_cK T} +\Psi ,
%     \end{align}
% where 
% \begin{align}
%     \Psi 
%     &= \frac{1}{C} [
%      \frac{5\eta_c^2KL^2}{2}(\sigma_c^2 +4KA^2) + \frac{\eta_s\eta_c L}{2}\sigma^2 +20L^2K^2\gamma^2\eta_c^2\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2] \, .
% \end{align}
% where $\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2=\sum_{i=1}^N\left(p_i^{avg}-p_i\right)^2 / p_i$ represents the chi-square divergence between the average aggragation weights $p^{avg}$ and the MAB aggregation weights $p$.
% \end{theorem}

% \begin{proof}
%     \begin{align}
% & E_t[{F}(w^{t+1})] \\
% & \overset{(a1)}{\leq} {F}(w^t) + \left \langle \nabla  {F}(w^t),E_t[w^{t+1}-w^t] \right \rangle + \frac{L}{2}E_t[\left \| w^{t+1}-w^t \right \|^2]  \\
% &= {F}(w^t)+\left \langle \nabla  {F}(w^t),E_t[\eta_s \Delta_t+\eta_s\eta_c K\nabla  {F}(w^t)-\eta_s\eta_c K \nabla  {F}(w^t)] \right \rangle+\frac{L}{2}\eta_s^2E_t[\left \|\Delta_t \right \|^2]  \\
% &=  {F}(w^t)-\eta_s\eta_c K\left \|\nabla  {F}(w^t)\right \|^2 + \eta_s\underbrace{\left \langle \nabla  {F}(w^t), E_t[\Delta_t+\eta_c K\nabla  {F}(w^t)] \right\rangle}_{P_1}+\frac{L}{2}\eta_s^2\underbrace{E_t\|\Delta_t\|^2}_{P_2} \, ,
% \end{align}

% \begin{align}
%     &\ P_1 \\
%    &=\left \langle \nabla  {F}(w^t),E_t[\Delta_t+\eta_cK\nabla  {F}(w^t)]\right\rangle   \\
%     &=\left \langle \nabla  {F}(w^t),E_t[-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\eta_cg_{i,k}^t+\eta_cK\nabla  {F}(w^t)]\right\rangle  \\
%     &\overset{(a2)}{=}\left \langle \nabla  {F}(w^t),E_t[-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\eta_c\nabla F_i(w_{i,k}^t)+\eta_cK\nabla  {F}(w^t)]\right\rangle  \\
%     &=\left \langle \sqrt{\eta_cK}\nabla  {F}(w^t),-\frac{\sqrt{\eta_c}}{\sqrt{K}}E_t[\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}(\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t))]\right\rangle  \\
%     &\overset{(a3)}{=}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2K}E_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}(\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t)) \right\|^2   \notag \\
%     &\ ~~~~ - \frac{\eta_c}{2 K}E_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \\
%     &\overset{(a4)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2}\sum_{k=0}^{K-1}\sum_{i=1}^Np^{avg}_i\mathbb{E}_t\left\|\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t) \right\|^2  \notag \\
%     &\ ~~~~- \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%      &\overset{(a5)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_cL^2}{2N}\sum_{i=1}^N\sum_{k=0}^{K-1}\mathbb{E}_t\left\|w_{i,k}^t-w^t \right\|^2 - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%     &\leq \left(\frac{\eta_cK}{2}+10K^3L^2\eta_c^3\gamma^2\right)\|\nabla  {F}(w^t)\|^2 + \frac{5L^2\eta_c^3}{2}K^2\sigma^2+  10\eta_c^3L^2K^3A^2  \notag \\ 
%     &\ ~~~~ - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \, ,
% \end{align}

% \begin{align}
%     &\ P_2 \\
%     &=\mathbb{E}_t\|\Delta_t\|^2   \\
%     &=\mathbb{E}_t\left\|\eta_c\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}g_{i,k}^t\right\|^2   \\
%     &=\eta_c^2\mathbb{E}_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}g_{i,k}^t-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2 +\eta_c^2\mathbb{E}_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2   \\
%     &\leq \eta_c^2\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\mathbb{E}\|g_i(w_{i,k}^t)-\nabla F_i(w_{i,k}^t)\|^2 +\eta_c^2\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%     & \overset{(a6)}{\leq} \eta_c^2K\sigma^2 
%     + \eta_c^2 \mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2    \, .
% \end{align}
% Now we take expectation over iteration on both sides of expression:
% \begin{align}
%     & \ F(w^{t+1}) \\
%     &\leq F(w^t)-\eta_s\eta_cK\mathbb{E}_t\left \|\nabla  {F}(w^t)\right \|^2 + \eta_s\mathbb{E}_t\left \langle \nabla  {F}(x^t),\Delta_t+\eta_cK\nabla  {F}(w^t) \right\rangle +\frac{L}{2}\eta_s^2\mathbb{E}_t\|\Delta_t\|^2   \\
%     &\overset{(a7)}{\leq} F(w^t) -\eta_s\eta_cK\left(\frac{1}{2}-20 L^2 K^2\eta_c^2\gamma^2(\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1) \right)\mathbb{E}_t\left\|\nabla  {f}(x_t)\right\|^2 
%     \notag \\ 
%     &\ ~~~~+\frac{5\eta_s\eta_c^3L^2K^2}{2}(\sigma^2 +4KA^2)  
%     +\frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 + 20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2  \notag \\
%     &\ ~~~~ -\left(\frac{\eta_s\eta_c}{2K}-\frac{L\eta_s^2\eta_c^2}{2}\right)\mathbb{E}_t\left\|\frac{1}{N}\sum_{i=1}^N\sum_{k=0}^{K-1}\nabla F_i(x_{i,k}^t)\right\|^2   \\
%     &\overset{(a8)}{\leq} F(w^t) -c\eta_s\eta_cK\mathbb{E}\left\|\nabla  {f}(x_t)\right\|^2 
%     +\frac{5\eta_s\eta_c^3L^2K^2}{2}(\sigma^2 +4KA^2)    \\
%     &\ ~~~~ +\frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 + 20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2  \notag \\
%     & \ ~~~~ -\left(\frac{\eta_s\eta_c}{2K}-\frac{L\eta_s^2\eta_c^2}{2}\right)\mathbb{E}_t\left\|\frac{1}{N}\sum_{i=1}^N\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2    \\
%     &\overset{(a9)}{\leq} F(w^t) - c\eta_s\eta_cK\mathbb{E}_t\|\nabla  {F}(w^t)\|^2 +\frac{5\eta_s\eta_c^3L^2K^2}{2}(\sigma^2 +4KA^2)  \notag \\
%     &\ ~~~~ + \frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 +20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2 \, ,
% \end{align}
% By recursively summing the the error difference above, we can obtain
% \begin{align}
%     \sum_{t=1}^{T-1}C\eta_s\eta_cK\mathbb{E}\|\nabla F(w^t)\|^2\leq F(w^0)-F(w^T)+T(\eta_s\eta_cK)\Psi,
% \end{align}
% where 
% \begin{align}
%     \Psi 
%     &= \frac{1}{C} [
%      \frac{5\eta_c^2KL^2}{2}(\sigma^2 +4KA^2) + \frac{\eta_s\eta_c L}{2}\sigma^2 +20L^2K^2\gamma^2\eta_c^2\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2] \, .
% \end{align}

% \begin{corollary}
%     Suppose $\eta_s$ and $\eta_c$ are $\eta_c=\mathcal{O}\left(\frac{1}{\sqrt{T}KL}\right)$ and $\eta_s=\mathcal{O}\left(\sqrt{KN}\right)$ such that the conditions mentioned above are satisfied. Then for sufficiently large T, the iterates of FedMABA satisfy:
%     \begin{align}
%         % \min_{t\in[T]}\mathbb{E}\|\nabla F(\boldsymbol{p^{avg}}^{(t)})\|^{2}\leq\mathcal{O}\left(\frac{F^0-F^*}{\sqrt{NKT}}\right)+\mathcal{O}\left(\frac{4\sqrt{N}\sigma^{2}L}{\sqrt{KT}}\right)+ \nonumber \\
%         % \mathcal{O}\left(\frac{6NL^2(K-1)\sigma^{2}}{KT}\right)+\mathcal{O}\left(\frac{12NL^2(K-1)A^2}{T}\right) .
%         \min_{t\in[T]}\mathbb{E}\left\|\nabla f\left(\boldsymbol{p^{avg}}_t\right)\right\|^2\leq\mathcal{O}\left(\frac{1}{\sqrt{NKT}}+\frac{1}{T}\right).
%     \end{align}
% \end{corollary}
% % \begin{align}
% %     &\ A_1 \\
% %     &\overset{(a4)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2}\sum_{k=0}^{K-1}\sum_{i=1}^Np^{avg}_i\mathbb{E}_t\left\|\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t) \right\|^2  \notag \\
% %     &\ ~~~~- \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
% %      &\overset{(a5)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_cL^2}{2N}\sum_{i=1}^N\sum_{k=0}^{K-1}\mathbb{E}_t\left\|w_{i,k}^t-w^t \right\|^2 - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
% %     &\leq \left(\frac{\eta_cK}{2}+10K^3L^2\eta_c^3\gamma^2\right)\|\nabla  {F}(w^t)\|^2 + \frac{5L^2\eta_c^3}{2}K^2\sigma^2+  10\eta_c^3L^2K^3A^2  \notag \\ 
% %     &\ ~~~~ - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \, ,
% % \end{align}
% \end{proof}



==> t.tex <==
\section{Proof of Theorem 1}
\paragraph{Preliminaries}

\noindent \textbf{McDiarmid's Inequality} 

Let \( Z_1, \ldots, Z_m \) be independent random variables and let \( f: \mathcal{Z}^m \rightarrow \mathbb{R} \) be a function satisfying the bounded difference property, i.e., for all \( i \) and for all \( z_1, \ldots, z_m, z'_i \) in \( \mathcal{Z} \),
\[ |f(z_1, \ldots, z_{i-1}, z_i, z_{i+1}, \ldots, z_m) - f(z_1, \ldots, z_{i-1}, z'_i, z_{i+1}, \ldots, z_m)| \leq c_i, \]
where \( c_i \) are non-negative constants. Then, for any \( a > 0 \), the following inequality holds:
\[ \mathbb{P}\left( |f(Z_1, \ldots, Z_m) - \mathbb{E}[f(Z_1, \ldots, Z_m)]| \geq a \right) \leq 2 \exp\left( -\frac{2a^2}{\sum_{i=1}^{m} c_i^2} \right). \]

\noindent \textbf{Hoeffding's Inequality}

Let \( X_1, \ldots, X_n \) be independent random variables with \( X_i \) taking values in the interval \( [a_i, b_i] \) almost surely. Define \( \overline{X} = \frac{1}{n} \sum_{i=1}^{n} X_i \) and let \( \mu = \mathbb{E}[\overline{X}] \). Then, for any \( t > 0 \), the following inequality holds:
\[ \mathbb{P}(|\overline{X} - \mu| \geq t) \leq 2 \exp\left( -\frac{2nt^2}{\sum_{i=1}^{n} (b_i - a_i)^2} \right). \]

\begin{assumption}[Bounded Loss]
    \label{bounded loss}
    W.L.O.G. for client $i$, $\forall \xi_i^m, \xi_i^n$, there exists a constant $c$, such that $\lvert F_i(w, \xi_i^m) - F_i(w, \xi_i^n)\rvert<c$.
\end{assumption}

\begin{definition}[Rademacher Complexity]
    Let $\mathcal{F} = F \circ w \triangleq \{\xi \rightarrow F(w, \xi) \mid w \in \mathcal{W}\}$, for any given dataset of FL $S=(\xi^1, ..., \xi^n)$, the set of loss mappings is denoted as $\mathcal{F}_{\mid S} \triangleq \{(F(\xi^1), ..., F(\xi^n)) \mid F\in \mathcal{F} \}$, the Rademacher Complexity is then defined as follows:
    \begin{align}
        \mathcal{R}(\mathcal{F}_{\mid S}) = \frac{1}{N}\mathbb{E}_{\tau \sim \{\pm 1\}^n}\sup_w\sum_{i=1}^N \frac{1}{n_i}\sum_{j=1}^{n_i}\tau F_i(\xi_i^j),
    \end{align}
    where \(\tau\) has an equal probability of 0.5 of being either 1 or -1.
\end{definition}

\begin{definition}[Representation of Generalization Error]
Given the data distribution \( D \) and the training data \( S \), the representation of generalization error is defined as the supremum of the difference between the expected risk and the empirical risk over the hypothesis space $\mathcal{W}$. Formally, it is expressed as:
\begin{align}
    Rep_D(S; \mathcal{W}, \mathcal{F}) = \sup_{w \in \mathcal{W}} (F_D(w) - F_S(w)), 
\end{align}
where $F_{\mathcal{D}}(w)=\mathbb{E}_{\tilde{\xi} \sim\mathcal{D}}F(w, \tilde{\xi})$, and $F_S(w) = \frac{1}{\lvert S \rvert} \sum_{\xi \in S} F(w, \xi)$.

\end{definition}

\begin{lemma}
    \label{empirical}
    Consider a data distribution $\mathcal{D}$ and any train set $S$. $\mathbb{E}_{S \sim D}Rep_{\mathcal{D}(S; \mathcal{F})} \leq 2\mathbb{E}_{S \sim D}R(\mathcal{F_{\mid S}})$.
\end{lemma}

\begin{proof}
   Given any dataset $S=(\xi_1, \xi_2, ..., \xi_n) \sim \mathcal{D}$, $S'=(\xi_1^{'}, \xi_2^{'}, ..., \xi_n^{'}) \sim D $. 
\[
\begin{aligned}
    \mathbb{E}_S Rep_{\mathcal{D}}(S; \mathcal{W}, \mathcal{F})
    &= \mathbb{E}_S \left[ \sup_{w \in \mathcal{W}} \{ F_{\mathcal{D}}(w) - F_{\mathcal{S}}(w) \} \right], \\
    &= \mathbb{E}_S \left[ \sup_{w \in \mathcal{W}} \{ \mathbb{E}_{S'} [F_{S'}(w)] - F_{S}(w) \} \right], \\
    &= \mathbb{E}_{S,S^{'}}\operatorname*{sup}_{w\in\mathcal{W}}\{\frac{1}{n}\sum_{i=1}^{n}(F(\xi_{i}^{\prime})-F(\xi_{i}))\}, \\
    &= \mathbb{E}_{S,S^{'},\tau\sim\{\pm1\}^n}\sup_{w\in\mathcal{W}}\{\frac1n\sum_{i=1}^n(\tau_iF(\xi_i^{\prime})-\tau_iF(\xi_i))\}, \\
    &\leq\mathbb{E}_{S^{\prime},\tau}\sup_F\{\frac1n\sum_{i=1}^n\tau_iF(\xi_i^{\prime})\}+\mathbb{E}_{S,\tau}\sup_F\{\frac1n\sum_{i=1}^m\tau_iF(\xi_i)\}, \\
    &= 2R(\mathcal{F_{\mid S}})
\end{aligned}
\] 
\end{proof}




% \begin{lemma}
%     \label{lemma 1}
%     Assume $\forall \xi_m, \xi_n$, $\lvert F_i(w, \xi_m) - F_i(w, \xi_n)\rvert<c$. Define $ \text{Rep}(\mathcal{H}, S) \triangleq \sup_{w \in \mathcal{H}} \left(F_i(w, \xi_m) - \hat{F}_i(w)  \right), $ where $\mathcal{H}$ is the parameter hypothesis set and \( S \) is the sample space, then for $\forall \delta \in \left[0, 1\right]$, with probability of at least $1-\delta$:
%     \begin{align}
%         Rep(\mathcal{H},S)\leq\mathbb{E}_SRep(\mathcal{H},S)+c\sqrt{\frac{2\ln(2/\delta)}{N}}
%     \end{align}
% \end{lemma}

% \begin{lemma}
%     Define
%     \begin{align}
%         R(\mathcal{F}|_{S}) \triangleq \frac{1}{N}\mathbb{E}_{\tau\sim\{\pm1\}^{n_i}}\sup_{w}
%         \sum_{i=1}^N \frac{1}{n_i}\sum_{j=1}^{n_i}\tau_{i, j}F_i(w_i, \xi_j) .
%     \end{align}
%     Combine Lemma \ref{lemma 1}, for $\forall \delta \in \left[0, 1\right]$, with probability of at least $1-2\delta$:
%     \begin{align}
%         \frac{1}{N}\sum_{i=1}^N(F_i(w_i)-\hat{F}_i(w_i)) \leq 2 R(\mathcal{F}|_{S}) + 3c\sqrt{\frac{2\ln(2/\delta)}{N}}
%     \end{align}
% \end{lemma}

\begin{theorem}[Bounded Generalization Error]
    \label{bounded generalization error}
    Consider a FL system with N clients, and parameter hypothesis space $\mathcal{W}$. If Assumption \ref{bounded loss} holds. Then, for $\forall \delta \in \left[0, 1\right]$ with probability of at least $1-2\delta$, for $\forall w \in \mathcal{W}$, the generalization error can be upper bounded as:
    \begin{align}
        Rep_D(S; \mathcal{W}, \mathcal{F}) \leq 2\mathcal{R}(\mathcal{F}_{\mid S}) + 3c\sqrt{\frac{2\ln \frac{2}{\delta}}{N}}.
    \end{align}
\end{theorem}

\begin{proof}
    Let's start with McDiarmid's Inequality, let $f(S)=Rep_D(S;\mathcal{F})$, we have 
    \begin{align}
        \mathbb{P}\left(\mathrm{Rep}_{\mathcal{D}}(S;\mathcal{F})-\mathbb{E}[\mathrm{Rep}_{\mathcal{D}}(S;\mathcal{F})]\geq\epsilon\right)\leq 2\exp\left(-\frac{2\epsilon^2}{mc^2}\right).
    \end{align}
    Set $\delta=\exp{(-\frac{2\epsilon^2}{Nc^2})}$, we then have
    \begin{align}
        \epsilon=c\sqrt{\frac{2\ln(2/\delta)}N}, 
    \end{align}
    Next, we consider empirical Rademacher complexity.
    According to \ref{empirical}, with a probability of at least $1-\delta$, we can obtain 
    \begin{align}
        \label{combine1}
        Rep_{\mathcal{D}}(S;\mathcal{F})\leq2\mathbb{E}_{S}R(\mathcal{F}|_{S})+c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}
    Then consider $\mathbb{E}_{S}R(\mathcal{F}|_{S})$, given $c^\prime = \frac{c}{2}\sqrt{N}$, with a probability of at least $1-\delta$, we have
    \begin{align}
        \label{combine2}
        \mathbb{E}_SR(\mathcal{F}|_S)\leq R(\mathcal{F}|_S)+c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}
    Combine \ref{combine1} and \ref{combine2}, and thus with a probability of at least $1-2\delta$, we have
    \begin{align}
        Rep_{\mathcal{D}}(S;\mathcal{F})\leq2R(\mathcal{F}|_{S})+3c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}
\end{proof}


\begin{corollary}[Bounded Generalization Error]
    \label{extended theorem}
     Under the same conditions as Theorem \ref{bounded generalization error}, let S, D be the training set and generalization data distribution, $w_S = ERM_w(S) = argmin_{w\in \mathcal{W}}{F(w;S)}$, $w^* = argmin_{w\in \mathcal{W}}{F(w;D)}$. Then, for $\forall \delta \in \left[0, 1\right]$ with probability of at least $1-3\delta$, for $\forall w \in \mathcal{W}$, the generalization error can be bounded as:
    \begin{align}
        F_{\mathcal{D}}(w_S)-F_{\mathcal{D}}(w^*)\leq 2\sup_{w \in \mathcal{W}} Var(F)+4c\sqrt{\frac{2\ln(2/\delta)}{N}}, 
    \end{align} 
    where $Var(F) = \sqrt{\frac{1}{N}\sum_{i=1}^{N}(F_{i}(w)-\frac{1}{N}\sum_{i=1}^{N}F_{i}(w))^2}$.
\end{corollary}

\begin{proof}
    Denote $w_S, w^*$ as $w_S=ERM_{\mathcal W}(S)=\arg\min_{w\in\mathcal W}\{F_S(w)\}, w^*=\arg\min_{w\in\mathcal W}\{F_D(w)\}$.
    Then we can rewrite generalization error as
    \begin{align}
        &F_{\mathcal{D}}(w_{S})-F_{\mathcal{D}}(w^{*})=\underbrace{[F_{\mathcal{D}}(w_{S})-F_{S}(w_{S})]}_{P_1}+\underbrace{[F_{S}(w_{S})-F_{S}(w^{*})]}_{P_2}+\underbrace{[F_{S}(w^{*})-F_{\mathcal{D}}(w^{*})]}_{P_3}.
    \end{align}

    \begin{align}
        \label{P1}
        P_1 &= F_{\mathcal{D}}(w_{S})-F_{S}(w_{S}) \\
        & \leq Rep_{\mathcal{D}}(S;\mathcal{F})\leq^{1-2\delta}2R(\mathcal{F}|_{S})+3c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}

    \begin{align}
        \label{P2}
        P_2 &= F_{S}(w_{S})-F_{S}(w^{*}) \\
        & \leq0.
    \end{align}

    According to the McDiarmid's inequality.
    \begin{align}
        \label{P3}
        F_{S}(w^{*})-F_{\mathcal{D}}(w^{*})\leq^{1-\delta}\frac{2c}{\sqrt{m}}\sqrt{\frac{m\ln(2/\delta)}{2}}.
    \end{align}

    Combining \ref{P1} to \ref{P3}, and following \cite{yuan2023equitable}, with a probability of at least $1-3\delta$, we obtain
    \begin{align}
        F_{\mathcal{D}}(w_S)-F_{\mathcal{D}}(w^*)\leq2\sup\limits_{w\in\mathcal{W}}Var(F)+4c\sqrt{\frac{2\ln(2/\delta)}{N}}.
    \end{align}    
\end{proof}

\section{Derivations of the Update Rule for the Player}
We mainly refer \cite{mao2021banditmtl} to the iterative derivation of $p$. We introduce the Legendre function related to $p$ as $\Phi_p(p)=\sum_{i=1}^Np_i\log p_i$. Assume the mirror gradient ascent step $t+1$, without loss of generality, in the dual space is $q^{t+1}$. The mirror gradient ascent step of the dual space can be defined as follows:
\begin{align}
    \label{all nabla}
    \nabla\Phi_p(q^{t+1})=\nabla\Phi_p(p^t)+\eta_b\mathbf{F}(w^t) ,
\end{align}
where $\mathbf{F}(w^t)$ denotes the loss vector of all participants, $\eta_b$ is the step size of the dual space, also known as MAB step size in main paper. For any client $i$, the corresponding $i$-th element of $\nabla\Phi_p(q^{t+1})$ is:
\begin{align}
    \label{element nabla}
    \nabla\Phi_p(q_i^{t+1})=1+\log q_i^{t+1} .
\end{align}
Combining \ref{all nabla} and \ref{element nabla}, the representational relationship between $q$ and $p$ is deduced as:
\begin{align}
    \label{q}
    q_i^{t+1}=e^{(\nabla\Phi_p(p_i^t)+\eta_bF_i(w_i^t)-1)}.
\end{align}
After updating the dual space weights $q^t$, in order to map them back to the original problem space to get update of $p^t$, we need to solve the following problem:
\begin{align}
    \label{map back}
    p^{t+1}=\arg\min_{p\in\mathcal{P}_{\rho,\mathbf{N}}}D_{\Phi_{p}}(p,q^{t+1}) ,
\end{align}
where $D_{\Phi_{p}}(p,q^{t+1}) = \Phi_p(p)-\Phi_p(q^{t+1})-\langle\nabla\Phi_p(q^{t+1}),p-q^{t+1}\rangle $ is the Bregman Divergence.

Incorporating the constraints of $p$, we establish the Lagrangian function as follows:
\begin{align}
&F(p^{t+1},\beta,\lambda)=\sum_{i=1}^{N}p_{i}^{t+1}\log\frac{p_{i}^{t+1}}{q_{i}^{t+1}} \nonumber \\ 
&- \beta(\sum_{i=1}^Np_i^{t+1}-1)-\lambda(\rho-\sum_{i=1}^Np_i^{t+1}\log p_i^{t+1}N).
\end{align}
Using the first order conditions, we have
\begin{align}
    p_i^{t+1}=(q_i^{t+1})^{\frac{1}{1+\lambda}}N^{-\frac{\lambda}{1+\lambda}}\exp(\frac{\alpha}{1+\lambda}-1).
\end{align}
Combining with $\sum_{i=1}^{N}p_{i}^{t+1}=1$, the constant part can be replaced by 
\begin{align}
    N^{-\frac\lambda{1+\lambda}}\exp\left(\frac\alpha{1+\lambda}-1\right)=\frac1{\sum_{i=1}^N(q_i^{t+1})^{\frac1{1+\lambda}}}, 
\end{align}
and then we have
\begin{align}
    \label{p iter}
    p_i^{t+1}=(q_i^{t+1})^{\frac{1}{1+\lambda}}/(\sum_{i=1}^N(q_i^{t+1})^{\frac{1}{1+\lambda}}).
\end{align}
By substituting \ref{p iter} back into the Lagrangian function and taking the derivative with respect to lambda, we have
\begin{align}
    \label{lambda diff}
    \frac{d}{d\lambda}\mathcal{L}(\lambda)&=\log N-\rho-\log\sum_{i=1}^N(q_i^{t+1})^{\frac1{1+\lambda}}\nonumber \\&- \frac{\sum_{i=1}^Nlog(q_i^{t+1})(q_i^{t+1})^{\frac1{1+\lambda}}}{(1+\lambda)\sum_{i=1}^N(q_i^{t+1})^{\frac1{1+\lambda}}}.
\end{align}
Combining \ref{lambda diff} and \ref{q}, the update formula for $p$ can be expressed as
\begin{align}
    p_i^{t+1}=\frac{e^{\frac{1}{1+\lambda^*}(\log p_i^t+\eta_bF_i(w^t_i)}}{\sum_{i=1}^Ne^{\frac{1}{1+\lambda^*}(\log p_i^t+\eta_bF_i(w^t_i)}}, 
\end{align}
where $\lambda^*$ is the kernel of $\frac{d}{d\lambda}\mathcal{L}(\lambda)$ which is denoted as $f(\lambda)$ in the main paper.

\section{Convergence of FedMABA}

\noindent Recall the assumptions we've made to derivate the convergence of FedMABA:
\begin{assumption}[Smoothness]
    \label{ass 1}
    Each objective function of clients is Lipschitz smooth, that is, there exists a constant $L > 0$, such that $\|\nabla F_i(\boldsymbol{x})-\nabla F_i(\boldsymbol{y})\|\leq L\left\|\boldsymbol{x}-\boldsymbol{y}\right\|,\forall i\in\{1,2,\ldots,N\}.$
\end{assumption}

\begin{assumption}[Unbiased Gradient and Bounded clients' Variance]
    \label{ass 2}
    The stochastic gradient calculated by each client can be an unbiased estimator of the clients' gradient $\mathbb{E}_\xi[g_i(\boldsymbol{p^{avg}}|\xi)]=\nabla F_i(\boldsymbol{p^{avg}}),$ and has bounded variance $\mathbb{E}_\xi[\|g_i(\boldsymbol{p^{avg}}|\xi)-\nabla F_i(\boldsymbol{p^{avg}})\|^2]\leq\sigma^2,\forall i\in\{1,2,\ldots,N\},\sigma^2\geq0.$
\end{assumption}

\begin{assumption}[Bounded Dissimilarity of Clients' Gradient]
    \label{ass 3}
    For any sets of weights $\{p_{i}^t\geq0\}_{i=1}^{N},\sum_{i=1}^{N}p_{i}^t=1,$, there exist constants $(\gamma^2+1) \geq 1$, $A^2 \geq 1$, such that $\sum_{i=1}^Np_i^t\left\|\nabla F_i(\boldsymbol{p^{avg}})\right\|^2\leq\gamma^2\left\|\sum_{i=1}^Np_i^t\nabla F_i(\boldsymbol{p^{avg}})\right\|^2+A^2.$
\end{assumption}

\begin{assumption}[Bounded Weights Divergence]
    \label{ass 4}
    For any sets of weights $p^t$ derived by FedMABA, $\chi_{p^a\|p^t}^{2}$, the chi-square divergence of $p^t$ and the average weights $p^a = \left[\frac{1}{N}, ..., \frac{1}{N}\right]$ can be upper bounded by $\kappa$, that is, $\forall t = 1, ..., T$, there exists a constant $\kappa$, such that $\chi_{p^a\|p^t}^{2} \leq \kappa$, where $\chi^2_{{p^a}\|{p^t}}=\sum_{i=1}^N\left(p^a_i-p^t_i\right)^2/p^t_i$.     
\end{assumption}


\noindent We first explain the gradient differences caused by the aggregation probability bias, following \cite{wang2020tackling}.

\begin{lemma}[Including bias in the error bound.]
    For any model parameter $w$, the difference between the gradients of $F^{avg}(w)=\sum_{i=1}^N p^{avg}_i F_i(w_i)$ and $F(w)=\sum_{i=1}^N p_i F_i(w_i)$ can be bounded as follows:
\begin{align}
    \|\nabla f^{avg}(w)-\nabla f(w)\|^2 \leq \chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2\left[(\gamma^2-1)\|\nabla {f}(w)\|^2+A^2 \right] \, ,
\end{align}
where $\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2$ denotes the chi-square distance between $\boldsymbol{p^{avg}}$ and $\boldsymbol{p}$, i.e., $\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2=\sum_{i=1}^N\left(p^{avg}_i-p_i\right)^2 / p_i$. $f(x)$ is the global objective with $f(w)=\sum_{i=1}^Np_if_i(w)$ where $\boldsymbol{p^{avg}}$ is usually the data ratio of clients. ${f}(w)=\sum_{i=1}^{N}p_if_i(w)$ is the  objective function of FedMABA with the reweight aggregation probability $\boldsymbol{p}$.
\label{objective gap}
\end{lemma}

\begin{proof}

\begin{equation}
\begin{aligned}
\nabla f^{avg}(x)-\nabla  {f}(\boldsymbol{x}) & =\sum_{i=1}^N\left(p^{avg}_i-p_i\right) \nabla f^{avg}_i(w) \\
& =\sum_{i=1}^N\left(p_i^{avg}-p_i\right)\left(\nabla f^{avg}_i(w)-\nabla  {f}(w)\right) \\
& =\sum_{i=1}^M \frac{p_i^{avg}-p_i}{\sqrt{p}_i} \cdot \sqrt{p}_i\left(\nabla f^{avg}_i(w)-\nabla {f}(w)\right) \, .
\end{aligned}
\end{equation}

Applying Cauchy-Schwarz inequality, it follows that
\begin{equation}
\begin{aligned}
\|\nabla f^{avg}(w)-\nabla {f}(w)\|^2 & \leq\left[\sum_{i=1}^N \frac{\left(p^{avg}_i-p_i\right)^2}{p_i}\right]\left[\sum_{i=1}^N p_i\left\|\nabla f^{avg}_i(w)-\nabla {f}(w)\right\|^2\right] \\
& \leq \chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2\left[(\gamma^2-1)\|\nabla {f}(w)\|^2+A^2\right] \, ,
\end{aligned}
\end{equation}
where the last inequality uses Assumption~\ref{ass 3}.
Note that
\begin{equation}
\begin{aligned}
\|\nabla f^{avg}(w)\|^2 & \leq 2\|\nabla f^{avg}(w)-\nabla {f}(w)\|^2+2\|\nabla {f}(w)\|^2 \\
& \leq 2\left[\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1\right]\|\nabla {f}(w)\|^2+2 \chi_{\boldsymbol{p^{avg}}\| \boldsymbol{p}}^2  A^2 \, .
\end{aligned}
\end{equation}

As a result, we obtain

\begin{align}
\min _{t \in[T]}\left\|\nabla f^{avg}\left(w^t\right)\right\|^2 & \leq \frac{1}{T} \sum_{t=0}^{T-1}\left\|\nabla f^{avg}\left(w^t\right)\right\|^2   \\
& \leq 2\left[\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1\right] \frac{1}{T} \sum_{t=0}^{T-1}\left\|\nabla {f}\left(w^t\right)\right\|^2+2 \chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2 A^2  \\
& \leq 2\left[\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1\right] \epsilon_{\mathrm{opt}}+2 \chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2 A^2 \, ,
\label{global convergence}
\end{align}
where $\epsilon_{\mathrm{opt}}= \frac{1}{T} \sum_{t=0}^{T-1}\left\|\nabla {f}\left(w^t\right)\right\|^2$ denotes the optimization error.
\end{proof}


\noindent Following \cite{wang2023delta}, we present the following convergence analysis.
\begin{lemma}[Local updates bound.]
    For a sufficiently small client's step size $\eta_c \leq \frac{1}{8LK}$, the local updates can be bounded as:
    \begin{align}
        \mathbb{E}\|w_{i,k}^t-w^t\|^2\leq20K^2(\eta_c^2\sigma^2+\eta_c^2A^2 + \gamma^2\eta_c^2\|\nabla F(x^t)\|^2).
    \end{align}
\end{lemma}

\begin{proof}

\begin{align}
    \mathbb{E}_t \|w_{i,k}^t-w^t\|^2 & = \mathbb{E}_t\|w_{i,k-1}^t-w^t-\eta_cg_{i,k-1}^t\|^2 \\
    & = \mathbb{E}_t\|w_{i,k-1}^t-w^t-\eta_c ( g_{i,k-1}^t-\nabla F_i(w_{i,k-1}^t)+\nabla F_i(w_{t,k-1}^t) -\nabla F_i(w^t)+\nabla F_i(w^t) ) \|^2 \\
    &\leq (1+\frac{1}{2K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\mathbb{E}_t\|\eta_c(g_{i,k-1}^t-\nabla F_i(w_{i,k}^t))\|^2 \notag \\
    &\quad +2K \mathbb{E}_t[\|\eta_L(\nabla F_i(w_{i,K-1}^t)-\nabla F_i(w^t))\|^2] + 2K\eta_c^2\mathbb{E}_t\|\nabla F_i(w^t)\|^2 \\
    &\leq (1+\frac{1}{2K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\eta_c^2\sigma^2 + 2K\eta_c^2L^2\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 \notag \\
    &\quad + 2K\eta_c^2A^2 + 2K\gamma^2\|\eta_c\nabla f(w^t)\|^2 \\
    &\leq (1+\frac{1}{K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\eta_c^2\sigma^2 + 2K\eta_c^2A^2 + 2K\gamma^2\|\eta_c\nabla F(w^t)\|^2 . 
\end{align}

By recursively applying the above formula, we can obtain,
\begin{align}
\mathbb{E}_t\|w_{i,k}^t-w^t\|^2 &\leq \sum_{p=0}^{k-1}(1+\frac{1}{K-1})^p\left[4K\eta_c^2\sigma^2+4K\eta_c^2A^2+4K\gamma^2\|\eta_c\nabla {F}(w^t)\|^2\right]  \\
&\leq (K-1)\left[(1+\frac{1}{K-1})^K-1\right]\left[4K\eta_c^2\sigma^2+4K\eta_c^2A^2+4K\gamma^2\|\eta_c\nabla {F}(w^t)\|^2\right]  \\
&\leq 20K^2(\gamma^2\eta_c^2\|\nabla {F}(w^t)\|^2 +\eta_c^2\sigma^2+\eta_c^2A^2)\, .
\end{align}
\end{proof}

We thus can formulate the convergence analysis of FedMABA.
\begin{theorem}[Convergence bound]
    Under Assumption \ref{ass 1} to \ref{ass 4}, let $\eta_s, \eta_c$ be the server updating step size, and the clinet's one, respectively. Set $\eta_c$ small enough as $\eta_c < \min (\frac{1}{8LK}, C)$, where C is a constant, such that $\frac{1}{2}-10 L^2\frac{1}{N}\sum_{i=1}^N K^2\eta_c^2\gamma^2(\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2)-1)^2+1) \leq c \leq 0$, and $\eta_s < \frac{1}{\eta_cL}$, the expectation of the gradient norm can be upper bounded when running FedMABA as:
    \begin{align}
    \mathop{min}_{\limits_{t\in[T]}} \mathbb{E}_t \|\nabla F(w^t)\|^2 \leq \frac{F^0-F^*}{c\eta_s\eta_cK T} +\Psi ,
    \end{align}
where 
\begin{align}
   \Psi 
    &= \frac{1}{C} [
     10\eta_c^2K^2L^2(\sigma^2 + A^2) + \frac{\eta_s\eta_c L}{2}\sigma^2 +20L^2K^2\gamma^2\eta_c^2\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2] \, .
\end{align}
where $\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2=\sum_{i=1}^N\left(p_i^{avg}-p_i\right)^2 / p_i$ represents the chi-square divergence between the average aggragation weights $p^{avg}$ and the MAB aggregation weights $p$.
\end{theorem}

\begin{proof}
    \begin{align}
& E_t[{F}(w^{t+1})] \\
& \overset{(a1)}{\leq} {F}(w^t) + \left \langle \nabla  {F}(w^t),E_t[w^{t+1}-w^t] \right \rangle + \frac{L}{2}E_t[\left \| w^{t+1}-w^t \right \|^2]  \\
&= {F}(w^t)+\left \langle \nabla  {F}(w^t),E_t[\eta_s \Delta_t+\eta_s\eta_c K\nabla  {F}(w^t)-\eta_s\eta_c K \nabla  {F}(w^t)] \right \rangle+\frac{L}{2}\eta_s^2E_t[\left \|\Delta_t \right \|^2]  \\
&=  {F}(w^t)-\eta_s\eta_c K\left \|\nabla  {F}(w^t)\right \|^2 + \eta_s\underbrace{\left \langle \nabla  {F}(w^t), E_t[\Delta_t+\eta_c K\nabla  {F}(w^t)] \right\rangle}_{P_1}+\frac{L}{2}\eta_s^2\underbrace{E_t\|\Delta_t\|^2}_{P_2} \, ,
\end{align}

\begin{align}
    &\ P_1 
    =\left \langle \nabla  {F}(w^t),E_t[\Delta_t+\eta_cK\nabla  {F}(w^t)]\right\rangle   \\
    &=\left \langle \nabla  {F}(w^t),E_t[-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\eta_cg_{i,k}^t+\eta_cK\nabla  {F}(w^t)]\right\rangle  \\
    &\overset{(a2)}{=}\left \langle \nabla  {F}(w^t),E_t[-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\eta_c\nabla F_i(w_{i,k}^t)+\eta_cK\nabla  {F}(w^t)]\right\rangle  \\
    &=\left \langle \sqrt{\eta_cK}\nabla  {F}(w^t),-\frac{\sqrt{\eta_c}}{\sqrt{K}}E_t[\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}(\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t))]\right\rangle  \\
    &\overset{(a3)}{=}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2K}E_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}(\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t)) \right\|^2   \notag \\
    &\ ~~~~ - \frac{\eta_c}{2 K}E_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \\
    &\overset{(a4)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2}\sum_{k=0}^{K-1}\sum_{i=1}^Np^{avg}_i\mathbb{E}_t\left\|\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t) \right\|^2  \notag \\
    &\ ~~~~- \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
     &\overset{(a5)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_cL^2}{2N}\sum_{i=1}^N\sum_{k=0}^{K-1}\mathbb{E}_t\left\|w_{i,k}^t-w^t \right\|^2 - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
    &\leq \left(\frac{\eta_cK}{2}+10K^3L^2\eta_c^3\gamma^2\right)\|\nabla  {F}(w^t)\|^2 + 10L^2\eta_c^3K^3\sigma^2+  10\eta_c^3L^2K^3A^2  \notag \\ 
    &\ ~~~~ - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \, ,
\end{align}

\begin{align}
    &\ P_2 
    =\mathbb{E}_t\|\Delta_t\|^2   \\
    &=\mathbb{E}_t\left\|\eta_c\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}g_{i,k}^t\right\|^2   \\
    &=\eta_c^2\mathbb{E}_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}g_{i,k}^t-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2 +\eta_c^2\mathbb{E}_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2   \\
    &\leq \eta_c^2\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\mathbb{E}\|g_i(w_{i,k}^t)-\nabla F_i(w_{i,k}^t)\|^2 +\eta_c^2\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
    & \overset{(a6)}{\leq} \eta_c^2K\sigma^2 
    + \eta_c^2 \mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2    \, .
\end{align}
Now we take expectation over iteration on both sides of expression:
\begin{align}
    & \ F(w^{t+1}) \\
    &\leq F(w^t)-\eta_s\eta_cK\mathbb{E}_t\left \|\nabla  {F}(w^t)\right \|^2 + \eta_s\mathbb{E}_t\left \langle \nabla  {F}(w^t),\Delta_t+\eta_cK\nabla  {F}(w^t) \right\rangle +\frac{L}{2}\eta_s^2\mathbb{E}_t\|\Delta_t\|^2   \\
    &\overset{(a7)}{\leq} F(w^t) -\eta_s\eta_cK\left(\frac{1}{2}-20 L^2 K^2\eta_c^2\gamma^2(\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1) \right)\mathbb{E}_t\left\|\nabla  {f}(w^t)\right\|^2 
    \notag \\ 
    &\ ~~~~+10\eta_s\eta_c^3L^2K^3(\sigma^2 +A^2)  
    +\frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 + 20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2  \notag \\
    &\ ~~~~ -\left(\frac{\eta_s\eta_c}{2K}-\frac{L\eta_s^2\eta_c^2}{2}\right)\mathbb{E}_t\left\|\frac{1}{N}\sum_{i=1}^N\sum_{k=0}^{K-1}\nabla F_i(x_{i,k}^t)\right\|^2   \\
    &\overset{(a8)}{\leq} F(w^t) -C\eta_s\eta_cK\mathbb{E}\left\|\nabla  {f}(w^t)\right\|^2 
    +10\eta_s\eta_c^3L^2K^3(\sigma^2 +A^2)    \\
    &\ ~~~~ +\frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 + 20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2  \notag \\
    & \ ~~~~ -\left(\frac{\eta_s\eta_c}{2K}-\frac{L\eta_s^2\eta_c^2}{2}\right)\mathbb{E}_t\left\|\frac{1}{N}\sum_{i=1}^N\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2    \\
    &\overset{(a9)}{\leq} F(w^t) - c\eta_s\eta_cK\mathbb{E}_t\|\nabla  {F}(w^t)\|^2 +10\eta_s\eta_c^3L^2K^3(\sigma^2 +A^2)  \notag \\
    &\ ~~~~ + \frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 +20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2 \, ,
\end{align}
By recursively summing the the error difference above, we can obtain
\begin{align}
    \sum_{t=1}^{T-1}C\eta_s\eta_cK\mathbb{E}\|\nabla F(w^t)\|^2\leq F(w^0)-F(w^T)+T(\eta_s\eta_cK)\Psi,
\end{align}
where 
\begin{align}
    \Psi 
    &= \frac{1}{C} [
     10\eta_c^2K^2L^2(\sigma^2 + A^2) + \frac{\eta_s\eta_c L}{2}\sigma^2 +20L^2K^2\gamma^2\eta_c^2\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2] \, .
\end{align}

\begin{corollary}
    Suppose $\eta_s$ and $\eta_c$ are $\eta_c=\mathcal{O}\left(\frac{1}{\sqrt{T}KL}\right)$ and $\eta_s=\mathcal{O}\left(\sqrt{KN}\right)$ such that the conditions mentioned above are satisfied. Then for sufficiently large T, the iterates of FedMABA satisfy:
    \begin{align}
        % \min_{t\in[T]}\mathbb{E}\|\nabla F(\boldsymbol{p^{avg}}^{(t)})\|^{2}\leq\mathcal{O}\left(\frac{F^0-F^*}{\sqrt{NKT}}\right)+\mathcal{O}\left(\frac{4\sqrt{N}\sigma^{2}L}{\sqrt{KT}}\right)+ \nonumber \\
        % \mathcal{O}\left(\frac{6NL^2(K-1)\sigma^{2}}{KT}\right)+\mathcal{O}\left(\frac{12NL^2(K-1)A^2}{T}\right) .
        \min_{t\in[T]}\mathbb{E}\left\|\nabla f\left(w\right)\right\|^2\leq\mathcal{O}\left(\frac{1}{\sqrt{NKT}}+\frac{1}{T}\right).
    \end{align}
\end{corollary}
% \begin{align}
%     &\ A_1 \\
%     &\overset{(a4)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2}\sum_{k=0}^{K-1}\sum_{i=1}^Np^{avg}_i\mathbb{E}_t\left\|\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t) \right\|^2  \notag \\
%     &\ ~~~~- \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%      &\overset{(a5)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_cL^2}{2N}\sum_{i=1}^N\sum_{k=0}^{K-1}\mathbb{E}_t\left\|w_{i,k}^t-w^t \right\|^2 - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%     &\leq \left(\frac{\eta_cK}{2}+10K^3L^2\eta_c^3\gamma^2\right)\|\nabla  {F}(w^t)\|^2 + \frac{5L^2\eta_c^3}{2}K^2\sigma^2+  10\eta_c^3L^2K^3A^2  \notag \\ 
%     &\ ~~~~ - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \, ,
% \end{align}
\end{proof}
% \noindent Following \cite{wang2023delta}, we present the following convergence analysis.
% \begin{lemma}[Local updates bound.]
%     For a sufficiently small client's step size $\eta_c \leq \frac{1}{8LK}$, the local updates can be bounded as:
%     \begin{align}
%         \mathbb{E}\|w_{i,k}^t-w^t\|^2\leq5K(\eta_c^2\sigma^2+4K\eta_c^2A^2)+20K^2\gamma^2\eta_c^2\|\nabla F(x^t)\|^2.
%     \end{align}
% \end{lemma}

% \begin{proof}

% \begin{align}
%     \mathbb{E}_t \|w_{i,k}^t-w^t\|^2 & = \mathbb{E}_t\|w_{i,k-1}^t-w^t-\eta_cg_{i,k-1}^t\|^2 \\
%     & = \mathbb{E}_t\|w_{i,k-1}^t-w^t-\eta_c ( g_{i,k-1}^t-\nabla F_i(w_{i,k-1}^t)+\nabla F_i(w_{t,k-1}^t) -\nabla F_i(w^t)+\nabla F_i(w^t) ) \|^2 \\
%     &\leq (1+\frac{1}{2K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\mathbb{E}_t\|\eta_c(g_{i,k-1}^t-\nabla F_i(w_{i,k}^t))\|^2 \notag \\
%     &\quad +2K \mathbb{E}_t[\|\eta_L(\nabla F_i(w_{i,K-1}^t)-\nabla F_i(w^t))\|^2] + 2K\eta_c^2\mathbb{E}_t\|\nabla F_i(w^t)\|^2 \\
%     &\leq (1+\frac{1}{2K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\eta_c^2\sigma^2 + 2K\eta_c^2L^2\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 \notag \\
%     &\quad + 2K\eta_c^2A^2 + 2K\gamma^2\|\eta_c\nabla f(w^t)\|^2 \\
%     &\leq (1+\frac{1}{K-1})\mathbb{E}_t\|w_{i,k-1}^t-w^t\|^2 + 2K\eta_c^2\sigma^2 + 2K\eta_c^2A^2 + 2K\gamma^2\|\eta_c\nabla F(w^t)\|^2 . 
% \end{align}

% By recursively applying the above formula, we can obtain,
% \begin{align}
% \mathbb{E}_t\|w_{i,k}^t-w^t\|^2 &\leq \sum_{p=0}^{k-1}(1+\frac{1}{K-1})^p\left[4K\eta_c^2\sigma^2+4K\eta_c^2A^2+4K\gamma^2\|\eta_c\nabla {F}(w^t)\|^2\right]  \\
% &\leq (K-1)\left[(1+\frac{1}{K-1})^K-1\right]\left[4K\eta_c^2\sigma^2+4K\eta_c^2A^2+4K\gamma^2\|\eta_c\nabla {F}(w^t)\|^2\right]  \\
% &\leq 20K^2(\gamma^2\eta_c^2\|\nabla {F}(w^t)\|^2 +\eta_c^2\sigma^2+\eta_c^2A^2)\, .
% \end{align}
% \end{proof}

% We thus can formulate the convergence analysis of FedMABA.
% \begin{theorem}[Convergence bound]
%     Under Assumption \ref{ass 1} to \ref{ass 4}, let $\eta_s, \eta_c$ be the server updating step size, and the clinet's one, respectively. Set $\eta_c$ small enough as $\eta_c < \min (\frac{1}{8LK}, C)$, where C is a constant, such that $\frac{1}{2}-10 L^2\frac{1}{N}\sum_{i=1}^N K^2\eta_c^2\gamma^2(\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2+1) \leq c \leq 0$, and $\eta_s < \frac{1}{\eta_cL}$, the expectation of the gradient norm can be upper bounded when running FedMABA as:
%     \begin{align}
%     \mathop{min}_{\limits_{t\in[T]}} \mathbb{E}_t \|\nabla F(w^t)\|^2 \leq \frac{F^0-F^*}{c\eta_s\eta_cK T} +\Psi ,
%     \end{align}
% where 
% \begin{align}
%     \Psi 
%     &= \frac{1}{C} [
%      \frac{5\eta_c^2KL^2}{2}(\sigma_c^2 +4KA^2) + \frac{\eta_s\eta_c L}{2}\sigma^2 +20L^2K^2\gamma^2\eta_c^2\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2] \, .
% \end{align}
% where $\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2=\sum_{i=1}^N\left(p_i^{avg}-p_i\right)^2 / p_i$ represents the chi-square divergence between the average aggragation weights $p^{avg}$ and the MAB aggregation weights $p$.
% \end{theorem}

% \begin{proof}
%     \begin{align}
% & E_t[{F}(w^{t+1})] \\
% & \overset{(a1)}{\leq} {F}(w^t) + \left \langle \nabla  {F}(w^t),E_t[w^{t+1}-w^t] \right \rangle + \frac{L}{2}E_t[\left \| w^{t+1}-w^t \right \|^2]  \\
% &= {F}(w^t)+\left \langle \nabla  {F}(w^t),E_t[\eta_s \Delta_t+\eta_s\eta_c K\nabla  {F}(w^t)-\eta_s\eta_c K \nabla  {F}(w^t)] \right \rangle+\frac{L}{2}\eta_s^2E_t[\left \|\Delta_t \right \|^2]  \\
% &=  {F}(w^t)-\eta_s\eta_c K\left \|\nabla  {F}(w^t)\right \|^2 + \eta_s\underbrace{\left \langle \nabla  {F}(w^t), E_t[\Delta_t+\eta_c K\nabla  {F}(w^t)] \right\rangle}_{P_1}+\frac{L}{2}\eta_s^2\underbrace{E_t\|\Delta_t\|^2}_{P_2} \, ,
% \end{align}

% \begin{align}
%     &\ P_1 \\
%    &=\left \langle \nabla  {F}(w^t),E_t[\Delta_t+\eta_cK\nabla  {F}(w^t)]\right\rangle   \\
%     &=\left \langle \nabla  {F}(w^t),E_t[-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\eta_cg_{i,k}^t+\eta_cK\nabla  {F}(w^t)]\right\rangle  \\
%     &\overset{(a2)}{=}\left \langle \nabla  {F}(w^t),E_t[-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\eta_c\nabla F_i(w_{i,k}^t)+\eta_cK\nabla  {F}(w^t)]\right\rangle  \\
%     &=\left \langle \sqrt{\eta_cK}\nabla  {F}(w^t),-\frac{\sqrt{\eta_c}}{\sqrt{K}}E_t[\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}(\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t))]\right\rangle  \\
%     &\overset{(a3)}{=}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2K}E_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}(\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t)) \right\|^2   \notag \\
%     &\ ~~~~ - \frac{\eta_c}{2 K}E_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \\
%     &\overset{(a4)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2}\sum_{k=0}^{K-1}\sum_{i=1}^Np^{avg}_i\mathbb{E}_t\left\|\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t) \right\|^2  \notag \\
%     &\ ~~~~- \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%      &\overset{(a5)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_cL^2}{2N}\sum_{i=1}^N\sum_{k=0}^{K-1}\mathbb{E}_t\left\|w_{i,k}^t-w^t \right\|^2 - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%     &\leq \left(\frac{\eta_cK}{2}+10K^3L^2\eta_c^3\gamma^2\right)\|\nabla  {F}(w^t)\|^2 + \frac{5L^2\eta_c^3}{2}K^2\sigma^2+  10\eta_c^3L^2K^3A^2  \notag \\ 
%     &\ ~~~~ - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \, ,
% \end{align}

% \begin{align}
%     &\ P_2 \\
%     &=\mathbb{E}_t\|\Delta_t\|^2   \\
%     &=\mathbb{E}_t\left\|\eta_c\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}g_{i,k}^t\right\|^2   \\
%     &=\eta_c^2\mathbb{E}_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}g_{i,k}^t-\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2 +\eta_c^2\mathbb{E}_t\left\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2   \\
%     &\leq \eta_c^2\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\mathbb{E}\|g_i(w_{i,k}^t)-\nabla F_i(w_{i,k}^t)\|^2 +\eta_c^2\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
%     & \overset{(a6)}{\leq} \eta_c^2K\sigma^2 
%     + \eta_c^2 \mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2    \, .
% \end{align}
% Now we take expectation over iteration on both sides of expression:
% \begin{align}
%     & \ F(w^{t+1}) \\
%     &\leq F(w^t)-\eta_s\eta_cK\mathbb{E}_t\left \|\nabla  {F}(w^t)\right \|^2 + \eta_s\mathbb{E}_t\left \langle \nabla  {F}(x^t),\Delta_t+\eta_cK\nabla  {F}(w^t) \right\rangle +\frac{L}{2}\eta_s^2\mathbb{E}_t\|\Delta_t\|^2   \\
%     &\overset{(a7)}{\leq} F(w^t) -\eta_s\eta_cK\left(\frac{1}{2}-20 L^2 K^2\eta_c^2\gamma^2(\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2(\gamma^2-1)+1) \right)\mathbb{E}_t\left\|\nabla  {f}(x_t)\right\|^2 
%     \notag \\ 
%     &\ ~~~~+\frac{5\eta_s\eta_c^3L^2K^2}{2}(\sigma^2 +4KA^2)  
%     +\frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 + 20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2  \notag \\
%     &\ ~~~~ -\left(\frac{\eta_s\eta_c}{2K}-\frac{L\eta_s^2\eta_c^2}{2}\right)\mathbb{E}_t\left\|\frac{1}{N}\sum_{i=1}^N\sum_{k=0}^{K-1}\nabla F_i(x_{i,k}^t)\right\|^2   \\
%     &\overset{(a8)}{\leq} F(w^t) -c\eta_s\eta_cK\mathbb{E}\left\|\nabla  {f}(x_t)\right\|^2 
%     +\frac{5\eta_s\eta_c^3L^2K^2}{2}(\sigma^2 +4KA^2)    \\
%     &\ ~~~~ +\frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 + 20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2  \notag \\
%     & \ ~~~~ -\left(\frac{\eta_s\eta_c}{2K}-\frac{L\eta_s^2\eta_c^2}{2}\right)\mathbb{E}_t\left\|\frac{1}{N}\sum_{i=1}^N\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\right\|^2    \\
%     &\overset{(a9)}{\leq} F(w^t) - c\eta_s\eta_cK\mathbb{E}_t\|\nabla  {F}(w^t)\|^2 +\frac{5\eta_s\eta_c^3L^2K^2}{2}(\sigma^2 +4KA^2)  \notag \\
%     &\ ~~~~ + \frac{\eta_s^2\eta_c^2KL}{2}\sigma^2 +20L^2K^3\gamma^2\eta_s\eta_c^3\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2 \, ,
% \end{align}
% By recursively summing the the error difference above, we can obtain
% \begin{align}
%     \sum_{t=1}^{T-1}C\eta_s\eta_cK\mathbb{E}\|\nabla F(w^t)\|^2\leq F(w^0)-F(w^T)+T(\eta_s\eta_cK)\Psi,
% \end{align}
% where 
% \begin{align}
%     \Psi 
%     &= \frac{1}{C} [
%      \frac{5\eta_c^2KL^2}{2}(\sigma^2 +4KA^2) + \frac{\eta_s\eta_c L}{2}\sigma^2 +20L^2K^2\gamma^2\eta_c^2\chi_{\boldsymbol{p^{avg}} \| \boldsymbol{p}}^2A^2] \, .
% \end{align}

% \begin{corollary}
%     Suppose $\eta_s$ and $\eta_c$ are $\eta_c=\mathcal{O}\left(\frac{1}{\sqrt{T}KL}\right)$ and $\eta_s=\mathcal{O}\left(\sqrt{KN}\right)$ such that the conditions mentioned above are satisfied. Then for sufficiently large T, the iterates of FedMABA satisfy:
%     \begin{align}
%         % \min_{t\in[T]}\mathbb{E}\|\nabla F(\boldsymbol{p^{avg}}^{(t)})\|^{2}\leq\mathcal{O}\left(\frac{F^0-F^*}{\sqrt{NKT}}\right)+\mathcal{O}\left(\frac{4\sqrt{N}\sigma^{2}L}{\sqrt{KT}}\right)+ \nonumber \\
%         % \mathcal{O}\left(\frac{6NL^2(K-1)\sigma^{2}}{KT}\right)+\mathcal{O}\left(\frac{12NL^2(K-1)A^2}{T}\right) .
%         \min_{t\in[T]}\mathbb{E}\left\|\nabla f\left(\boldsymbol{p^{avg}}_t\right)\right\|^2\leq\mathcal{O}\left(\frac{1}{\sqrt{NKT}}+\frac{1}{T}\right).
%     \end{align}
% \end{corollary}
% % \begin{align}
% %     &\ A_1 \\
% %     &\overset{(a4)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_c}{2}\sum_{k=0}^{K-1}\sum_{i=1}^Np^{avg}_i\mathbb{E}_t\left\|\nabla F_i(w_{i,k}^t)-\nabla F_i(w^t) \right\|^2  \notag \\
% %     &\ ~~~~- \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
% %      &\overset{(a5)}{\leq}\frac{\eta_cK}{2}\|\nabla  {F}(w^t)\|^2+\frac{\eta_cL^2}{2N}\sum_{i=1}^N\sum_{k=0}^{K-1}\mathbb{E}_t\left\|w_{i,k}^t-w^t \right\|^2 - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2   \\
% %     &\leq \left(\frac{\eta_cK}{2}+10K^3L^2\eta_c^3\gamma^2\right)\|\nabla  {F}(w^t)\|^2 + \frac{5L^2\eta_c^3}{2}K^2\sigma^2+  10\eta_c^3L^2K^3A^2  \notag \\ 
% %     &\ ~~~~ - \frac{\eta_c}{2 K}\mathbb{E}_t\|\sum_{i=1}^Np^{avg}_i\sum_{k=0}^{K-1}\nabla F_i(w_{i,k}^t)\|^2 \, ,
% % \end{align}
% \end{proof}
